Learning Neural Light Fields with Ray-Space Embedding Networks

Neural radiance fields (NeRFs) produce state-of-the-art view synthesis results. However, they are slow to render, requiring hundreds of network evaluations per pixel to approximate a volume rendering integral. Baking NeRFs into explicit data structures enables efficient rendering, but results in a large increase in memory footprint and, in many cases, a quality reduction. In this paper, we propose a novel neural light field representation that, in contrast, is compact and directly predicts integrated radiance along rays. Our method supports rendering with a single network evaluation per pixel for small baseline light field datasets and can also be applied to larger baselines with only a few evaluations per pixel. At the core of our approach is a ray-space embedding network that maps the 4D ray-space manifold into an intermediate, interpolable latent space. Our method achieves state-of-the-art quality on dense forward-facing datasets such as the Stanford Light Field dataset. In addition, for forward-facing scenes with sparser inputs we achieve results that are competitive with NeRF-based approaches in terms of quality while providing a better speed/quality/memory trade-off with far fewer network evaluations.

==> figures/fig_embedding_vis.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/figure_4a}\hfill
(a) Epipolar Image and Predicted Image without embedding \\[3mm]
\includegraphics[width=\linewidth]{figures/figure_4b}
\raggedright
(b) Embedding visualization (left) and predicted image and EPI (right) \\[3mm]



\caption{
\tb{Embedding Facilitates Light Field Learning}. (a) Without embedding, an MLP learns a severely distorted EPI and heldout views. (b) An embedding network facilitates light field learning by allowing for better registration and interpolation. Note that color level sets in the EPI (right) correspond to the same rays with similar embeddings (left).
}
\label{fig:affine_motivation}
\vspace{-5mm}
\end{figure}


==> figures/fig_qual.tex <==
\begin{figure}[t]
\footnotesize
\centering%
%
	% \mpage{0.35}{%
	% 	\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/0005_pred_ours.png}\\%
	% 	\emph{Horns}
	% }%
	% \hspace{-1mm}\hfill%
	% \mpage{0.64}{%
	% 	\mpage{0.24}{%
	% 		\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup1_005_gt.png}\\[0.2mm]%
	% 		\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup2_005_gt.png}\\[-1mm]%
	% 		XX\,dB%
	% 	}\hspace{-1mm}\hfill%
	% 	\mpage{0.24}{%
	% 		\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup1_005_pred_nerf.png}\\[0.2mm]%
	% 		\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup2_005_pred_nerf.png}\\[-1mm]%
	% 		XX\,dB%
	% 	}\hspace{-1mm}\hfill%
	% 	\mpage{0.24}{%
	% 		\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup1_0005_pred_ours.png}\\[0.2mm]%
	% 		\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup2_0005_pred_ours.png}\\[-1mm]%
	% 		XX\,dB%
	% 	}\hspace{-1mm}\hfill%
	% 	\mpage{0.24}{%
	% 		\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup1_0005_pred_teacher.png}\\[0.2mm]%
	% 		\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup2_0005_pred_teacher.png}\\[-1mm]%
	% 		XX\,dB%
	% 	}%
	% }%
%
	\mpage{0.35}{%
		\begin{overpic}[width=\linewidth]{figures/results/qual/horns_compare/0005_pred_ours.png}%
			\put(18, 62){\Large\color{red}$\Box$}%
			\put(62, 38){\Large\color{red}$\Box$}%
		\end{overpic}\\[-0.5mm]%
		\emph{Horns}
	}%
	\hspace{-1mm}\hfill%
	\mpage{0.64}{%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup1_005_gt.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup2_005_gt.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup1_005_pred_nerf.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup2_005_pred_nerf.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup1_0005_pred_ours.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup2_0005_pred_ours.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup1_0005_pred_teacher.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/horns_compare/closeup2_0005_pred_teacher.png}%
		}%
	}\\[1mm]%
%
	\mpage{0.35}{%
		\begin{overpic}[width=\linewidth]{figures/results/qual/trex_compare/0005_pred_ours.png}%
			\put(15, 10){\Large\color{red}$\Box$}%
			\put(52, 1){\Large\color{red}$\Box$}%
		\end{overpic}\\[-0.5mm]%
		\emph{T-Rex}
	}%
	\hspace{-1mm}\hfill%
	\mpage{0.64}{%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/trex_compare/closeup1_005_gt.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/trex_compare/closeup2_005_gt.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/trex_compare/closeup1_005_nerf.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/trex_compare/closeup2_005_nerf.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/trex_compare/closeup1_0005_pred_ours.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/trex_compare/closeup2_0005_pred_ours.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/trex_compare/closeup1_0005_pred_teacher.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/trex_compare/closeup2_0005_pred_teacher.png}%
		}%
	}\\[1mm]%
%
	\mpage{0.35}{%
		\begin{overpic}[width=\linewidth]{figures/results/qual/flower_compare/0000_pred_ours.png}%
			\put(56, 45){\Large\color{red}$\Box$}%
			\put(1, 63){\Large\color{red}$\Box$}%
		\end{overpic}\\[-0.5mm]%
		\emph{Flower}
	}%
	\hspace{-1mm}\hfill%
	\mpage{0.64}{%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/flower_compare/closeup1_000_gt.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/flower_compare/closeup2_000_gt.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/flower_compare/closeup1_000_pred_nerf.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/flower_compare/closeup2_000_pred_nerf.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/flower_compare/closeup1_0000_pred_ours.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/flower_compare/closeup2_0000_pred_ours.png}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			\includegraphics[width=\linewidth]{figures/results/qual/flower_compare/closeup1_0000_pred_teacher.png}\\[0.2mm]%
			\includegraphics[width=\linewidth]{figures/results/qual/flower_compare/closeup2_0000_pred_teacher.png}%
		}%
	}\\[1mm]%
%
	\mpage{0.35}{%
	}%
	\hspace{-1mm}\hfill%
	\mpage{0.64}{%
		\mpage{0.24}{%
			GT%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			NeRF~\cite{mildenhall2020nerf}%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			Ours (w/o teacher)%
		}\hspace{-1mm}\hfill%
		\mpage{0.24}{%
			Ours (w/ teacher)%
		}%
	}\\[-2mm]%
%
\caption{%
\tb{Visual comparisons on sparse light fields.} (\emph{left}) We show our view synthesis results of Real Forward-Facing scenes. (\emph{right}) The close-ups reveal our representation leads to more faithful reconstruction of view dependent effects (``Horns'' and ``T-Rex'') and sharper results (``Flower''). See our \emph{supplementary material} for more results on both Real Forward-Facing and Stanford scenes.
}%
%
\label{fig:qual}
\vspace{-5mm}
\end{figure}

